Language-Guided Joint Audio-Visual Editing via One-Shot Adaptation

In this paper, we introduce a novel task called language-guided joint audio-visual editing. Given an audio and image pair of a sounding event, this task aims at generating new audio-visual content by editing the given sounding event conditioned on the language guidance. For instance, we can alter the background environment of a sounding object while keeping its appearance unchanged, or we can add new sounds contextualized to the visual content. To address this task, we propose a new diffusion-based framework for joint audio-visual editing and introduce two key ideas. Firstly, we propose a one-shot adaptation approach to tailor generative diffusion models for audio-visual content editing. With as few as one audio-visual sample, we jointly transfer the audio and vision diffusion models to the target domain. After fine-tuning, our model enables consistent generation of this audio-visual sample. Secondly, we introduce a cross-modal semantic enhancement approach. We observe that when using language as content editing guidance, the vision branch may overlook editing requirements. This phenomenon, termed catastrophic neglect, hampers audio-visual alignment during content editing. We therefore enhance semantic consistency between language and vision to mitigate this issue. Extensive experiments validate the effectiveness of our method in language-based audio-visual editing and highlight its superiority over several baseline approaches. We recommend that readers visit our project page for more details: https://liangsusan-git.github.io/project/avedit/.

==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/intro_backup.tex <==
\vspace{-8pt}
\section{Introduction}
\label{sec:intro}
When we see an accordion and hear its sound, can we imagine it being played in different settings? Picturize it being played on a rainy day with the rainfall sounds in the background. What would it sound like in a large hall? We answer these questions by proposing a new language-guided audio-visual personalization task. Given a few audio and image pairs of an object that emits sound, the goal of this task is to learn the unique auditory as well as visual features of the object, and synthesize new audio-visual content in various contexts while maintaining the object's unique characteristics. As shown in Fig.~\ref{fig:teaser}, this new task learns specific concepts of an accordion and generates new audio-visual samples of the same accordion based on different prompts, \textit{e.g.}, \textit{a person playing the accordion on a rainy day}. 
This novel task enhances user experience by personalizing multimedia content according to individual preferences.
%The new task enhances user experience and satisfaction by tailoring multimedia content to the user's preferences.

%Personalization is a key topic in the machine learning community, where some researchers develop training strategies to improve the visual reconstruction capabilities of generative models \cite{DBLP:journals/tog/BauSPWZZ019,roich2022pivotal,alaluf2022hyperstyle,cao2022authentic,nitzan2022mystyle}, and some works focus on achieving customization in recommendation systems \cite{cho2002personalized,martinez2009s,amat2018artwork,benhamdi2017personalized}. 
Very recently, several diffusion-based works \cite{text-inversion,dreambooth,custom-diffusion,animate-a-story} have been proposed to address the vision personalization problem. For instance, the Textual Inversion method \cite{text-inversion} inverses the visual feature of an object to a learnable token. DreamBooth \cite{dreambooth} employs a special and rarely appeared identifier to represent the target object. Although these methods make significant advancements in their respective areas, no existing approach manages to solve the language-based audio-visual personalization problem.

Audio-visual personalization requires jointly memorizing the auditory and visual characteristics of a sounding object. Existing personalization approaches \cite{text-inversion,dreambooth} only enable unimodal personalization. A naive extension of unimodal customization methods to the audio-visual task would isolate the audio modeling and the vision modeling, harming the audio-visual consistency of synthesized samples. To overcome this challenge, we introduce a novel multi-modal conditional embedding, which bridges the gap between two modalities. The multi-modal conditional embedding learns a joint representation of the audio and visual attributes of a sounding object. The learned representation effectively enhances the quality and audio-visual correlation of generated content.

%Instead of utilizing  We extract explicit semantic information from audio and image pairs, and fuse audio information with vision information to generate a joint audio-visual representation of the new content. The generated audio-visual representation is then projected into the text embedding space as textual conditions. Our method enhances the semantic expressiveness of the textual token and enables cross-modal diffusion control.

Moreover, the language-based audio-visual personalization problem calls for language-guided creation of audio-visual content. When using the same prompt for guiding both audio and image generation, the discrepancy in text understanding hinders the generation quality.  The audio generation focuses on the audio information implied by a text prompt, such as sound content, audio effects, melody, and rhythm, while the image generation relies on the visual cues indicated in the prompt, including appearance, shape, geometry, and texture. This misalignment in text comprehension can result in mismatched audio-visual content. Therefore, we design a Large Language Model-assisted (LLM) prompt refinement approach to settle this problem. We utilize the text reasoning capabilities of the LLM to generate the audio-sensitive prompt and vision-sensitive prompt based on the user's instruction. We complement two prompts with cross-modal information to align them semantically. The processed prompts improve the audio-visual correlation of synthesized content and enhance language control over content creation.

%The user's prompt is used as a guide for controlling the audio-visual synthesis. 

%While these methods advance image customization, a naive application of these approaches to audio-visual personalization does not yield optimal results because (1) these methods learn an implicit, non-semantic textual representation of a user-provided concept. (2) These personalization approaches demand learning two isolated representations of an audio-visual concept for each audio and vision modality. (3) The image and audio personalization processes are separated from each other, leading to audio-visual content with low cross-modal semantic correlation. (4) There is a discrepancy in text understanding between audio diffusion models and vision diffusion models. Text models of each modality focus on different aspects of the same prompt.

%The advent of diffusion models sheds light on this problem, providing a new way to personalize audio-visual content. Diffusion models, especially text-to-image diffusion models \cite{imagen,dalle2,stablediffusion,controlnet,instructpix2pix}, show remarkable abilities in controllable content generation. These models, by leveraging the intricate relationships between textual semantics and visual content, can transform textual descriptions into vivid images. The success of text-to-image diffusion models inspires us to design a language-guided audio-visual personalization method based on diffusion models. We tune diffusion models to bind textual identifiers with user-provided audio-visual concepts, catering these powerful models to user preferences. Thanks to the text-conditional generation ability of diffusion models, we enable text-controlled and high-fidelity synthesis of audio-visual content.

%The advent of text-to-image diffusion models \cite{imagen,dalle2,stablediffusion,controlnet,instructpix2pix} has ushered in a new era of content generation, where textual descriptions can be transformed into vivid visual representations. These models, by leveraging the intricate relationships between textual semantics and visual content, have shown remarkable capabilities in generating high-quality images from textual prompts. However, as the field has evolved, there has been a growing interest in personalizing these generated outputs to cater to specific user preferences or to align with certain reference data.

%Several diffusion works \cite{text-inversion,dreambooth,custom-diffusion,animate-a-story} have proposed similar ideas to address the vision personalization problem. For instance, the Textual Inversion method \cite{text-inversion} encapsulates the new concept in a learnable token and composes the new token with different texts to generate new images. Synthesized images share the same concept with the reference images (e.g., a cat) but contain different contexts (e.g., a cat on the grass, a backpack with a cat painting). DreamBooth \cite{dreambooth} employs a special and rarely appeared identifier (e.g., sks) to represent the target concept. The identifier can guide the generation process, ensuring that the output aligns with the desired appearance or style. Because parameters of the diffusion model are updated during personalization training, which eases the optimization process, DreamBooth shows stronger personalization capability than Textual Inversion. Custom Diffusion \cite{custom-diffusion}, another notable approach, points out that the cross-attention layer has more significant weight changes than other the rest of the network during personalization fine-tuning. This work suggests only updating the key and value projection matrices to improve the fine-tuning efficiency.

%Several diffusion works \cite{text-inversion,dreambooth,custom-diffusion,animate-a-story} have proposed similar ideas to address the vision personalization problem. For instance, the Textual Inversion method \cite{text-inversion} encapsulates the new concept in a learnable token and composes the new token with different texts to generate new images. DreamBooth \cite{dreambooth} employs a special and rarely appeared identifier (e.g., sks) to represent the target concept. While these methods advance image customization, a naive application of these approaches to audio-visual personalization does not yield optimal results because (1) these methods learn an implicit, non-semantic textual representation of a user-provided concept. (2) These personalization approaches demand learning two isolated representations of an audio-visual concept for each audio and vision modality. (3) The image and audio personalization processes are separated from each other, leading to audio-visual content with low cross-modal semantic correlation. (4) There is a discrepancy in text understanding between audio diffusion models and vision diffusion models. Text models of each modality focus on different aspects of the same prompt.

%To overcome these problems, we introduce a novel multi-modal conditional embedding. We extract explicit semantic information from audio and image pairs, and fuse audio information with vision information to generate a joint audio-visual representation of the new content. The generated audio-visual representation is then projected into the text embedding space as textual conditions. Our method enhances the semantic expressiveness of the textual token and enables cross-modal diffusion control.

%Moreover, we design a Large Language Model-assisted (LLM) prompt refinement approach to settling the discrepancy in text understanding. We leverage LLM to parse a prompt into audio-related and vision-related prompts. Then, we complement words of each modality with cross-modal information to semantically align two prompts. In this way, we effectively handle the information redundancy and omission problems of user-provided prompts. 

Our work is the first to study the diffusion-based audio-visual personalization problem. Therefore, we collect an Audio-Visual Personalization (AVP) dataset of 30 audio-visual concepts to benchmark our method. We curate this dataset with instrument concepts and speech concepts, considering that these two classes are among the most common and easily recognizable sounding objects~\cite{audioset}. We believe the AVP dataset will lay the foundation for addressing more general and more complex sounding objects.

%The dataset includes 21 kinds of instrument concepts and 9 speech concepts. The instrument concepts range from woodwind instruments to percussion instruments, and the speech concepts cover various languages, genders, and races.

%significantly advanced the field of text-to-image synthesis, the realm of audio-visual learning remains relatively unexplored, especially in the context of personalization. Audio-visual learning \cite{owens2018audio,localization_easy,tian2018audio,soundspaces,semantic_navigation,sound_pixel,2.5D,zhou2020sep,guo2021ad,unicon,zhou2022avs,avnerf}, which involves the concurrent processing of both audio and visual data, offers a richer and more holistic understanding of content. The synergy between these two modalities can lead to more coherent and contextually relevant outputs. However, despite its potential, there has been no method that leverages this synergy for personalization purposes. To the best of our knowledge, we are the first to delve into the domain of audio-visual personalization.

%In this paper, we present a pioneering approach to audio-visual personalization using language-guided multi-modal diffusion models. Our method stands out by extracting unique multi-modal concepts from a few reference audio and image pairs and synthesizing new samples that retain the same concept but in varied contexts. Unlike previous methods that rely on learnable tokens or special identifiers, our approach introduces a novel multi-modal conditional embedding. This embedding generates textual tokens conditioned on reference audio-visual data, thereby enhancing the expressiveness of textual tokens with cross-modal information. Furthermore, to ensure the high fidelity of the generated samples, we incorporate a detail preservation method that capitalizes on the rich features of reference samples. This not only ensures personalized generation but also elevates the quality of the output.

Through extensive experiments, we demonstrate the proposed method can effectively address the challenges of the audio-visual personalization problem. Moreover, we showcase the versatility of our method by applying it to tasks like room acoustic adjustment and audio-visual composition.%, further emphasizing its potential in the realm of multi-modal personalization.
We summarize our contributions as follows:
\begin{itemize}
\item We introduce a new language-guided audio-visual personalization task, studying the customized generation of audio-visual content based on diffusion models.

\item We propose novel multi-modal conditional embeddings and LLM-assisted prompt refinement approach to achieve the correlated synthesis of audio-visual content.

\item We construct a new Audio-Visual Personalization dataset (AVP) that contains various audio-visual concepts for performance evaluation. Our method exhibits noticeable advantages over several existing baselines.

\item We showcase the application of our method in tasks such as room acoustic adjustment and audio-visual composition, highlighting its potential in diverse multi-modal personalization scenarios.

\end{itemize}

